An Optimal Dynamic Mechanism for Multi-Armed Bandit Processes

We consider the problem of revenue-optimal dynamic mechanism design in settings where agents' types evolve over time as a function of their (both public and private) experience with items that are auctioned repeatedly over an infinite horizon. A central question here is understanding what natural restrictions on the environment permit the design of optimal mechanisms (note that even in the simpler static setting, optimal mechanisms are characterized only under certain restrictions). We provide a {\em structural characterization} of a natural "separable: multi-armed bandit environment (where the evolution and incentive structure of the a-priori type is decoupled from the subsequent experience in a precise sense) where dynamic optimal mechanism design is possible. Here, we present the Virtual Index Mechanism, an optimal dynamic mechanism, which maximizes the (long term) {\em virtual surplus} using the classical Gittins algorithm. The mechanism optimally balances exploration and exploitation, taking incentives into account.

==> app_proofs.tex <==
\il{This is file is not currently in use to the be the best of my knowledge.}
\iffalse

\subsection{Omitted Proofs}

\begin{proof} [{\bf Proof of Lemma~\ref{lemma:monotone_q}}]
The proofs consists of showing that
both $\alpha_i$ and $\beta_i$ are non-decreasing functions of
$\theta_i$, under Assumption \ref{ass:weights}. With this it directly
follows that the Virtual index is monotonic in the initial reports.

In additive case, dropping the $i$ subscripts,
\[
\beta^\prime = \frac{\eta^\prime}{\eta^2} A^\prime -\frac{1}{\eta}A^{\prime\prime}
\]
where $(\cdot)^\prime$ denotes a derivative. Now by assumption, and
using that the hazard rate is non-negative, we have that the above
is non-negative.

In multiplicative case, first note that $\alpha =
1-\frac{1}{\eta}(\log A)^\prime$, so
\[
\alpha' = \frac{\eta^\prime}{\eta^2}\frac{A^\prime}{A} -
\frac{1}{\eta} (\log A)^{\prime \prime}
\]
which is non-negative (note that $A$ is non-negative). Since $\beta =(\alpha-1)C$
 and since $C$ is positive,
$\beta$ is non-decreasing.
\end{proof}


%\subsection{More proofs}  \label{app:separable}

\begin{proof} [{\bf proof of Lemma~\ref{lem:alapha_beta}}]
In the additively separable case, we
have:
\begin{eqnarray*}
\virtuali(\theta_i,\experience_i,\info_i)=
A_i(\theta_i,\info_i)+B_i(\experience_i,\info_i) -
\frac{1}{\eta_i(\theta_i)} A_i^\prime(\theta_i,\info_i)
\end{eqnarray*}
and the claim follows. In the multiplicatively separable case, we
have:
\begin{eqnarray*}
\virtuali(\theta_i,\experience_i,\info_i)  &= &
A_i(\theta_i)B_i(\experience_i,\info_i) -C_i(\info_i)-
\frac{1}{\eta_i(\theta_i)} A_i^\prime(\theta_i,\info_i)
B_i(\experience_i,\info_i) \\
&=&\left(A_i(\theta_i)-\frac{1}{\eta_i(\theta_i)} A_i^\prime(\theta_i,\info_i)\right)
B_i(\experience_i,\info_i) -C_i(\info_i)
 \\
&=&\alpha_i(\theta_i) A_i(\theta_i) B_i(\experience_i,\info_i) -C_i(\info_i)
 \\
&=&\alpha_i(\theta_i) \valuei(\theta_i,\experience_i,\info_i) +(\alpha_i(\theta_i)-1)C_i(\info_i)\\
&=&\alpha_i(\theta_i) \valuei(\theta_i,\experience_i,\info_i) +\beta_i(\theta_i,\info_i)
\end{eqnarray*}
and the claim follows.
\end{proof}



\begin{proof}[{\bf Proof of Lemma~\ref{lemma:vcg}}]
At each time $t$. Let $m_{i,t}$ denote the marginal contribution of agent $i$, at time $t$, to the virtual surplus.
%
$$m_{i,t} = W(\statet) - W_{-i}(\statet) - \delta \Expct[W(\statetplus) - W_{-i}(\statetplus)] $$

Note that if the mechanism does not allocate to $i$, then $m_{i,t}$ and also $p_{i,t,}$ are equal to $0$.
But, if the mechanism allocates the item to agent $i$ at time $t$.

\begin{eqnarray*}
m_{i,t} & = & W(\statet) - W_{-i}(\statet) - \delta \Expct[W(\statetplus) - W_{-i}(\statetplus)] \\
& = & \virtual_{i}(\thetaRiz, \thetaRit, \experienceit, \infoit) - (1-\delta) W_{-i}(\statet) \\
& = & \alpha_i(\thetaRiz) v_i(\thetaRit, \experienceit, \infoit) + \beta(\thetaRit, \infoit) -  (1-\delta)  W_{-i}(\statet)  \\
& = & \alpha_i(\thetaRiz) \left(v_i(\theta_i, \experienceit, \infoit) -  p_{i,t}\right)
\end{eqnarray*}
Hence, for the utility of agent $i$ we have:

$$U_{i}(\state) = {1\over\alpha_i(\thetaRiz)} \Expct[\sumt \deltat  m_i] = {1\over\alpha_i(\thetaRiz)} \left(W(\statet) - W_{-i}(\statet)\right) $$

Note that $W_{-i}(\state_{-i,t})$ is independent of agent $i$ reports.
Also, $W(\statet)$ is be maximized only if $i$ reports truthfully.
To show this, suppose agent $i$ deviates from the truthful strategy and chooses reporting strategy $R$.
The virtual surplus of the allocation induced by $R$ is less than or equal to $W(\statet)$.
Hence, $i$ is better off by not deviating.
\end{proof}




\begin{proof}[{\bf Proof of Lemma~\ref{lem:theta_IC}}]

Let $U_i(\theta)$ be the expected utility of $i$ in under the virtual
index mechanism conditioned on the initial types being $\theta$ (and
everyone behaving truthfully). First, we prove that ex poste periodic
IC holds. Note that by Lemma~\ref{lemma:vcg}, we only have to show
this for the $t=0$ timestep.

Let $\tilde U_i(\theta;\theta_i^\prime)$ be the utility of agent $i$
conditioned on: the initial types being $\theta$; the initial report
in the $0$-th period of $i$ being $\theta_i^\prime$; where $i$ behaves
optimally thereafter; and where all other agents behave truthfully
(conditioned on their initial type and report being $\theta_{-i}$). To
prove (periodic ex post) IC, we must show that for all $\theta$ and all
$\theta_i^\prime$ ,
\[
U_i(\theta) \geq \tilde U_i(\theta;\theta_i^\prime)
\]
(As we show IR later, we can assume that the report $\theta_i^\prime$ in the
0-th period has non-negative utility).

Let $\theta^\prime$ equal $\theta$ in all coordinates except in
coordinate $i$, where it equals $\theta_i^\prime$.
Lemma~\ref{lemma:vcg} shows that truthfulness is the
optimal continuation strategy from time $t\geq 1$ onwards.
Hence,
\[
U_i(\theta^\prime) = \tilde U_i(\theta^\prime;\theta_i^\prime)
\]
Thus, it suffices to show:
\begin{equation}\label{eq:suffices}
U_i(\theta)-U_i(\theta^\prime) \geq
\tilde U_i(\theta;\theta_i^\prime)-\tilde U_i(\theta^\prime;\theta_i^\prime)
\end{equation}
for all $\theta$ and $\theta_i^\prime$. Now we write this condition
more explicitly.

\sk{this is botched. the discounting at $t=0$ is the same as at $t=1$}.

By construction, we have that:
\begin{eqnarray*}
U_i(\theta)
&=& \gValuei(\theta) - (p_{i,0} + \Expct\left[\sumt \deltat q_{i,t} p_{i,t}  \middle\vert \theta \right] \\
&=& \gValuei(\theta) - \gPricei(\theta)\\
&=& \int_0^{\theta_i}
\Expct\left[\sumt \deltat \gallocit
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert \theta_i=z, \theta_{-i} \right] dz
\end{eqnarray*}
Here, we are slightly abusing
notation in that we only specifying the superscript with respect to $z$
in $\gallocit$ (it implicitly also depends on $\theta_{-i}$).

Now let us consider the mechanism $q^{\theta^\prime}(\cdot)$ from
$t\geq1$, where $\theta^\prime$ is fixed. Let
$U_i^{\theta^\prime}(\theta)$ be the utility of this mechanisms from
$t\geq 1$ onwards (where truthful reporting occurs).  By Lemma~\ref{lemma:vcg} , we have that $q^{\theta^\prime}$ is an
incentive compatible allocation.  Hence, the envelope
lemma implies:
\[
U_i^{\theta^\prime}(\theta)- U_i^{\theta^\prime}(\theta^\prime)
= \int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumt \delta^t \allocit^{\theta^\prime}
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert\theta_i=z,\theta_{-i}\right] dz
\]
Now note that at $t=0$ the charge only
depends on the initial report (e.g. $\theta^\prime$). Hence,
\[
\tilde U_i(\theta;\theta_i^\prime)-\tilde U_i(\theta^\prime;\theta_i^\prime)
=U_i^{\theta^\prime}(\theta)- U_i^{\theta^\prime}(\theta^\prime)
= \int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumt \deltat \allocit^{\theta^\prime}
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert\theta_i=z,\theta_{-i}\right] dz
\]
where now the evolution of the process is under the mechanism
$q^{\theta^\prime}$.

Using these two expressions, we have that Equation~\ref{eq:suffices}
is equivalent to:
\begin{align*}
\int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumt \deltat \gallocit
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert\theta_i=z,\theta_{-i}\right] dz
\geq \\
 \int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumt \deltat \allocit^{\theta^\prime}
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert z,\theta_{-i}\right] dz
\end{align*}
We can couple the two expectations by sampling the initial types and an
infinite sequence of experiences --- then each process is evolved on
this sample using the appropriate allocations. Thus, this condition is
equivalent to:
\begin{align*}
\int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumt \deltat \left(
\gallocit
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
-
\allocit^{\theta^\prime}
\frac{\partial \valuei(z,\experienceit^\prime,\infoit^\prime)}{\partial z}
\right)
\middle\vert \theta_i=z,\theta_{-i}\right] dz
\geq 0
\end{align*}
where $\experienceit^\prime$ and $\infoit^\prime$ denote the experiences under
the allocation $q^{\theta^\prime}$.

Now let $\tau_k$ be the time at which the $k$-th allocation occurs
under the $\gallocit$ (assumed to be infinite if the $k$-th allocation
does not occur), and let $\tau_k^\prime$ be this time under
$\allocit^{\theta^\prime}$. By our coupled process, we have that
$\experience_{i,\tau_k^\prime}^\prime$ equals $\experience_{i,\tau_k}$ for
all $k$. This is because after $k$ allocations, both private
experiences have advanced precisely $k-1$ times. Similarly, the
same is true for the public experiences. Hence, the above condition is
equivalent to:
\[
\int_{\theta_i^\prime}^{\theta_i}
\Expct\left[\sumk \left(
\delta^{\tau_k}
-
\delta^{\tau_k^\prime}
\right)
\frac{\partial \valuei(z,\experience_{i,\tau_k},\info_{i,\tau_k})}
{\partial z}
\middle\vert\theta_i=z,\theta_{-i} \right] dz
\]
since the experiences at $\tau_k$ and $\tau_k^\prime$ are identical.

To complete the proof of IC, we show that $\tau_k^\prime \geq \tau_k$,
using the monotonicity of the allocation
(Lemma~\ref{cond:monotone_q}). This implies that:
\[
q^{\theta^\prime}(z,\experience_t,\info_t) \leq
%q^{z}(z,\experience_t,\info_t)
= \galloc(z,\experience_t,\info_t) \, .
\]
We proceed inductively. For $k=1$, note that until the first
allocation occurs in either process, the state of $i$ is identical at
each timestep under both allocations --- this is because the Gittins
allocation is index mechanism (so the states of the other agents
advance identically when $i$ is not present). Hence, monotonicity
implies that the first allocation under $q^{\theta^\prime}$ cannot
occur before that time under $\galloc$. Taking the inductive step,
assume that $\tau_{k-1}^\prime \geq \tau_{k-1}$. If
$\tau_{k-1}^\prime\geq \tau_k$, then we are done. If not, this implies
at time $\tau_{k-1}^\prime$, agent $i$ has been allocated
precisely $k-1$ times in both processes, and so she has an identical
state in either process. Hence, an identical argument to that of the
first period shows that the $k$-th allocation (if it occurs) under
$q^{\theta^\prime}$ cannot occur before that under $\galloc$.


\sk{clean up argument of IR}

To complete the proof, we show that $\gmech$ is incentive
compatible and that $U_i^\gmech(\theta_i=0)=0$. By construction, the
expected cumulative payment by $i$, conditioned on $\theta$ is just
$\gPricei(\hat\theta)$, since the other terms cancel in
expectation. Hence, we have
that:
\begin{align*}
U_i^\gmech(\theta) &=
\gValuei(\theta)-\gPricei(\theta) \\
&=
\int_0^{\theta_i}
\Expct\left[\sumt \deltat \gallocit
\frac{\partial \valuei(z,\experienceit,\infoit)}{\partial z}
\middle\vert \theta_i=z, \theta_{-i} \right] dz \\
& \geq 0
\end{align*}
Also, note that this implies $U_i^\gmech(\theta_i=0)=0$. For all
subsequent rounds, we have IR by assumption on $\calM^{\rinit}$.
\end{proof}
\fi
